NSP-BERT: A Prompt-based Few-Shot Learner Through an Original Pre-training Task--Next Sentence Prediction

Using prompts to utilize language models to perform various downstream tasks, also known as prompt-based learning or prompt-learning, has lately gained significant success in comparison to the pre-train and fine-tune paradigm. Nonetheless, virtually all prompt-based methods are token-level, meaning they all utilize GPT's left-to-right language model or BERT's masked language model to perform cloze-style tasks. In this paper, we attempt to accomplish several NLP tasks in the zero-shot scenario using a BERT original pre-training task abandoned by RoBERTa and other models--Next Sentence Prediction (NSP). Unlike token-level techniques, our sentence-level prompt-based method NSP-BERT does not need to fix the length of the prompt or the position to be predicted, allowing it to handle tasks such as entity linking with ease. Based on the characteristics of NSP-BERT, we offer several quick building templates for various downstream tasks. We suggest a two-stage prompt method for word sense disambiguation tasks in particular. Our strategies for mapping the labels significantly enhance the model's performance on sentence pair tasks. On the FewCLUE benchmark, our NSP-BERT outperforms other zero-shot methods on most of these tasks and comes close to the few-shot methods.

==> figures/cse_nsp.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.85\columnwidth]{images/cse_nsp.pdf}

\caption{Conceptual comparison between End-to-End representation-based \textbf{\underline c}ontrastive learning of \textbf{\underline s}entence \textbf{\underline e}mbeddings (CSE) and All-to-All interaction-based \textbf{\underline n}ext \textbf{\underline s}entence \textbf{\underline p}rediction (NSP). Except that the output of the model is not the representation of the sentence, the NSP task uses a weak self-supervision method to train the BERT.}
\label{fg:cse_nsp}
\end{figure}

==> tables/soft_position.tex <==
\begin{table}[h]
    \center
    \renewcommand\arraystretch{1.0}
    \resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{llcc}
    \toprule
        \multirow{2}{*}{\bf ORG} & \multirow{2}{*}{\bf Models} & {\bf Hard-Position} & {\bf Soft-Position} \\
         &  & (Dev / Test) & (Dev / Test) \\ \midrule
        \multicolumn{1}{l|}{\multirow{1}{*}{\bf Google\cref{fn:google_bert}}} & \multicolumn{1}{l|}{BERT-Chinese} & {\bf 46.04} / 48.15 & 41.09 / {\bf 48.65↑} \\ \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-4}
        \multicolumn{1}{l|}{\multirow{2}{*}{\bf HFL\cref{fn:hfl}}} & \multicolumn{1}{l|}{BERT-wwm} & {\bf 46.53} / {\bf 47.56} & 45.05 / 46.05↓ \\ 
        \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{BERT-wwm-ext} & 51.49 / 52.90 & {\bf 53.47} / {\bf \underline{54.55↑}} \\ \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-4}
        \multicolumn{1}{l|}{\multirow{1}{*}{\bf UER\cref{fn:uer}}} & \multicolumn{1}{l|}{BERT-mixed} & 47.52 / 50.85 & {\bf 53.96} / {\bf 52.00↑} \\ \bottomrule
        %  & mixed-BERT & 56.44/51.30 & 38.12/38.61↓ \\ \hline
    \end{tabular}
    }
    \caption{Accuracy of NSP-BERT with soft-position compared with hard-position on cloze-style task ChID. The models we adopted are from different organizations. }
    \label{tb:soft_position}
\end{table}
\label{sec:soft_position}

==> tables/two_stage.tex <==
\begin{table}[h]
    \center
    \renewcommand\arraystretch{1.0}
    \resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{llcccc}
    \toprule
        \multirow{2}{*}{\bf ORG} & \multirow{2}{*}{\bf Models} & \multicolumn{2}{l|}{\bf Entity Linking} & \multicolumn{2}{l}{\bf Entity Typing} \\ 
         &  & One-S & \multicolumn{1}{l|}{Two-S} & One-S & Two-S \\ \midrule
        \multicolumn{1}{l|}{\multirow{1}{*}{\bf Google\cref{fn:google_bert}}} & \multicolumn{1}{l|}{BERT-Chinese} & 60.77 & \multicolumn{1}{l|}{\bf 66.99↑} & 24.08 & {\bf 31.18↑} \\ 
        \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-4} \cmidrule(r){5-6}
        \multicolumn{1}{l|}{\multirow{2}{*}{\bf HFL\cref{fn:hfl}}} & \multicolumn{1}{l|}{BERT-wwm} & 57.86 & \multicolumn{1}{l|}{\bf 66.64↑} & 23.99 & {\bf 28.64↑} \\ 
        \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{BERT-wwm-ext} & 59.03 & \multicolumn{1}{l|}{\bf 66.82↑} & 24.25 & {\bf 31.71↑} \\ 
        \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-4} \cmidrule(r){5-6}
        \multicolumn{1}{l|}{\multirow{1}{*}{\bf UER\cref{fn:uer}}} & \multicolumn{1}{l|}{BERT-mixed} & 61.16 & \multicolumn{1}{c|}{\bf \underline{69.66↑}} & 31.35 & {\bf 40.04↑} \\ \midrule
        \multicolumn{1}{l|}{\multirow{2}{*}{\bf Baselines}} & \multicolumn{1}{l|}{GPT-{\sc Zero}} & / & \multicolumn{1}{c|}{/} & \multicolumn{2}{c}{28.48} \\
        \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{PET-{\sc Zero}} & / & \multicolumn{1}{c|}{/} & \multicolumn{2}{c}{\underline{\bf 40.46}} \\
        
    \bottomrule
    \end{tabular}
    }
    \label{tb:two_stage}
    \caption{Results (Acc.) of NSP-BERT on DuEL2.0 with one-stage prompt (One-S) and two-stage prompt (Two-S). Since GPT-{\sc Zero} and PET-{\sc Zero} are hard to handle variable length entity description, we can not report their performance on entity linking.
    }
    \vspace{-6pt}
\end{table}
